A parton recombination approach to heavy ion collisions at RHIC and LHC

This thesis discusses the phenomenological parton recombination approach to describe hadronization in heavy ion collisions. The very good agreement to RHIC data for the flow coefficients v_2 and v_4 is shown and extrapolations are used to make predictions for the LHC.

==> babelbst.tex <==
%%
%% This is file `babelbst.tex',
%% generated with the docstrip utility.
%%
%% The original source files were:
%%
%% merlin.mbs  (with options: `bblbst')
%% 
%% IMPORTANT NOTICE:
%% 
%% For the copyright see the source file.
%% 
%% Any modified versions of this file must be renamed
%% with new filenames distinct from babelbst.tex.
%% 
%% For distribution of the original source see the terms
%% for copying and modification in the file merlin.mbs.
%% 
%% This generated file may be distributed as long as the
%% original source files, as listed above, are part of the
%% same distribution. (The sources need not necessarily be
%% in the same archive or directory.)
%% Copyright 1994-2004 Patrick W Daly
 % ===============================================================
 % IMPORTANT NOTICE:
 % This bibliographic style (bst) file has been generated from one or
 % more master bibliographic style (mbs) files, listed above.
 %
 % This generated file can be redistributed and/or modified under the terms
 % of the LaTeX Project Public License Distributed from CTAN
 % archives in directory macros/latex/base/lppl.txt; either
 % version 1 of the License, or any later version.
 % ===============================================================
 % Name and version information of the main mbs file:
 % \ProvidesFile{merlin.mbs}[2004/02/09 4.13 (PWD, AO, DPC)]
 % This is babelbst.tex for English.
 % It should serve as a model for other languages.
 % Alternatively, store it under a different name (e.g. englbst.tex)
 % and then \input it with a command in babelbst.tex.
\def\bbland{und}                \def\bbletal{et~al.}
\def\bbleditors{Herausgeber}        \def\bbleds{Hg.}
\def\bbleditor{Herausgeber}          \def\bbled{Hg.}
\def\bbledby{herausgegeben von}
\def\bbledition{Auf\/lage}        \def\bbledn{Aufl.}
\def\bblvolume{Band}          \def\bblvol{Bd.}
\def\bblof{von}
\def\bblnumber{Nummer}          \def\bblno{Nr.}
\def\bblin{in}
\def\bblpages{Seiten}            \def\bblpp{S.}
\def\bblpage{Seite}              \def\bblp{S.}
\def\bbleidpp{Seiten}
\def\bblchapter{Kapitel}        \def\bblchap{Kap.}
\def\bbltechreport{Technischer Bericht}
\def\bbltechrep{Techn.\ Ber.}
\def\bblmthesis{Diplomarbeit}
\def\bblphdthesis{Dissertation}
\def\bblfirst{Erste}            \def\bblfirsto{1.}
\def\bblsecond{Zweite}          \def\bblsecondo{2.}
\def\bblthird{Dritte}            \def\bblthirdo{3.}
\def\bblfourth{Vierte}          \def\bblfourtho{4.}
\def\bblfifth{F\^^b{u}nfte}            \def\bblfiftho{5.}
\def\bblst{.}  \def\bblnd{.}  \def\bblrd{.}
\def\bblth{.}
\def\bbljan{Januar}  \def\bblfeb{Februar}  \def\bblmar{M\^^b{a}rz}
\def\bblapr{April}    \def\bblmay{Mai}       \def\bbljun{Juni}
\def\bbljul{Juli}     \def\bblaug{August}    \def\bblsep{September}
\def\bbloct{Oktober}  \def\bblnov{November}  \def\bbldec{Dezember}
\endinput
%%
%% End of file `babelbst.tex'.

